Freetures: Localization in Signed Distance Function Maps

Localization of a robotic system within a previously mapped environment is important for reducing estimation drift and for reusing previously built maps. Existing techniques for geometry-based localization have focused on the description of local surface geometry, usually using pointclouds as the underlying representation. We propose a system for geometry-based localization that extracts features directly from an implicit surface representation: the Signed Distance Function (SDF). The SDF varies continuously through space, which allows the proposed system to extract and utilize features describing both surfaces and free-space. Through evaluations on public datasets, we demonstrate the flexibility of this approach, and show an increase in localization performance over state-of-the-art handcrafted surfaces-only descriptors. We achieve an average improvement of ~12% on an RGB-D dataset and ~18% on a LiDAR-based dataset. Finally, we demonstrate our system for localizing a LiDAR-equipped MAV within a previously built map of a search and rescue training ground.

==> archive.tex <==
\section{Archive}

\begin{table}
\centering
\ra{1.3}
\begin{tabular}{@{}rrrrrr@{}}
\toprule
\phantom{abc} & \phantom{abc} & \multicolumn{4}{c}{Dataset} \\
\cmidrule{3-6}
Method & Parameter & All & 3D & Carto & MAV \\
\midrule
FPFH~\cite{rusu2009fast}  & $r_f$ (m) & & 0.093 & 1.5 & 1.5 \\
                          & $r_n$ (m)  &  & 0.093 & 1.5 & 1.5 \\
                          & $k_\text{dist}$ (m) & & 0.05 & 0.5 & 0.5 \\
                          & \#NN  & 1 & & &  \\
\midrule
SHOT~\cite{salti2014shot} & $r_f$ (m) & & 0.186 & \red{1.5} & \red{1.5} \\
                          & $r_n$ (m)  & & 0.093 & 1.5 & 1.5 \\
                          & $k_\text{dist}$ (m) & & 0.05 & 0.5 & 0.5 \\
                          & \#NN  & 1 & & & \\
\midrule
Ours                      & $r_f$ (vox) & 15 \\
                          & div/$180^{\circ}$  & 10 \\
                          & \#NN      & 5  \\
                          & $\alpha_{\text{dist}}$  & $1e^{-7}$ \\
                          & $\alpha_{\text{class}}$ & $1e^{-5}$ \\
                          & $\sigma_{\text{grad}}$ (vox) & 2 \\
                          & $\sigma_{\text{desc}}$ (vox) & 15 \\
                          & $k_\text{dist}$ (m) & & 0.1 & 1.0 & 1.5 \\ 
\bottomrule
\end{tabular}
\caption{Critical parameters of the proposed and baseline methods. Parameters which are used in all evaluations described in Sections~\ref{sec:results_3dmatch}, \ref{sec:results_deutsches}, and \ref{sec:results_arche} are in column ``all'', while parameters changing between datasets have their respective values indicated in the columns ``3D'', ``Carto'', and ``MAV''.}
\label{tab:parameters}
% \vspace{-5mm}
\end{table}


% \begin{figure*}[t] %H_1
%     \centering
%     \begin{subfigure}[b]{0.22\textwidth}
%         \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=\columnwidth]{figures/sdf_vs_fpfh/dataset_1.png}
%         \label{fig:dm_1}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.22\textwidth}
%         \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=\columnwidth]{figures/sdf_vs_fpfh/dataset_2.png}
%         % \caption{}
%         \label{fig:dm_2}    
%     \end{subfigure}
%     \begin{subfigure}[b]{0.22\textwidth}
%         \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=\columnwidth]{figures/sdf_vs_fpfh/dataset_3.png}
%         \label{fig:dm_3}    
%     \end{subfigure}
%     \begin{subfigure}[b]{0.22\textwidth}
%         \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=\columnwidth]{figures/sdf_vs_fpfh/dataset_4.png}
%         \label{fig:dm_4}    
%     \end{subfigure}
%     \begin{subfigure}[b]{0.22\textwidth}
%         \includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=\columnwidth]{figures/sdf_vs_fpfh/dataset_5.png}
%         \label{fig:dm_5}
%     \end{subfigure}
%     \caption{Precision-Recall curves for the proposed method (blue) and a comparison method (red) (FPFH features). Maps are created using 3D lidar data from the Deutsches Museum dataset~\cite{hess2016real}.\todo{Need to find some way of displaying the maps.}}
%     \label{fig:precision_recall_curves}
%     % \vspace{-5mm}
% \end{figure*}
